FIRE: A Dataset for Feedback Integration and Refinement Evaluation of Multimodal Models

Vision language models (VLMs) have achieved impressive progress in diverse applications, becoming a prevalent research direction. In this paper, we build FIRE, a feedback-refinement dataset, consisting of 1.1M multi-turn conversations that are derived from 27 source datasets, empowering VLMs to spontaneously refine their responses based on user feedback across diverse tasks. To scale up the data collection, FIRE is collected in two components: FIRE-100K and FIRE-1M, where FIRE-100K is generated by GPT-4V, and FIRE-1M is freely generated via models trained on FIRE-100K. Then, we build FIRE-Bench, a benchmark to comprehensively evaluate the feedback-refining capability of VLMs, which contains 11K feedback-refinement conversations as the test data, two evaluation settings, and a model to provide feedback for VLMs. We develop the FIRE-LLaVA model by fine-tuning LLaVA on FIRE-100K and FIRE-1M, which shows remarkable feedback-refining capability on FIRE-Bench and outperforms untrained VLMs by 50%, making more efficient user-agent interactions and underscoring the significance of the FIRE dataset.

==> checklist.tex <==
\section*{Checklist} 

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See~\cref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The contributions and scope are claimed in the abstract and introduction.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, we have discussed the limitations in ~\cref{sec:conclusion}. }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, we have discussed the potential negative societal impacts of our work in the supplementary materials. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We ensure that our paper is fully conforming to the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{This paper does not include theoretical results. }
	\item Did you include complete proofs of all theoretical results?
     \answerNA{This paper does not include theoretical results. }
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and data can be found in the URL, \href{https://mm-fire.github.io}{\texttt{mm-fire.github.io}}. The detailed setting of experiments can be found in ~\cref{sec:experiment}. The prompts for generating the conversations are shown in the supplementary materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All the training details can be found in ~\cref{sec:experiment}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{The error bars for the student model and the teacher model are discussed in the supplementary materials.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The computing resources are included in ~\cref{sec:experiment}.}
    
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the creators of all the existing assets used in this paper.}
  \item Did you mention the license of the assets?
    \answerYes{We mentioned the license of the assets in the supplementary materials.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We did not include new assets in the supplemental material or as a URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All the data sources of this paper are public datasets. }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{All the data sources of this paper are public datasets, which did not include any personally identifiable information.  }
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No crowdsourcing and human subjects are involved in this paper. }
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{No crowdsourcing and human subjects are involved in this paper. }
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{No crowdsourcing and human subjects are involved in this paper. }
\end{enumerate}

\end{enumerate}

==> datasheet.tex <==
\section{Datasheet for FIRE}

We present a Datasheet \cite{gebru2021datasheets} for documentation and responsible usage of our internet knowledge databases. The required author statement, hosting, licensing, metadata, and maintenance plan can be found in the datasheet.

\subsection{Motivation}

\paragraph{For what purpose was the dataset created?} We create this large-scale dataset to facilitate research towards enhancing the feedback-reflecting ability of VLMs.

\paragraph{Who created the dataset (e.g., which team, research group) and on
behalf of which entity (e.g., company, institution, organization)?} This dataset was created by Pengxiang Li (Beijing Institute of Technology), Zhi Gao (BIGAI), Bofei Zhang (BIGAI), Tao Yuan (BIGAI), Yuwei Wu (Beijing Institute of Technology), Mehrtash Harandi (Monash University), Yunde Jia (Beijing Institute of Technology), Song-chun Zhu (BIGAI), Qing Li (BIGAI).

\subsection{Distribution}
\paragraph{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?} Yes, the dataset is publicly available on the internet.

\paragraph{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?}
The dataset can be downloaded from \url{https://huggingface.co/datasets/PengxiangLi/FIRE}. We use Creative Commons Attribution 4.0 License (CC BY 4.0). The Croissant metadata can be found on the dataset hosting platform (\url{https://huggingface.co/}).

\paragraph{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?} No.

\paragraph{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} No.

\subsection{Maintenance}
\paragraph{Who will be supporting/hosting/maintaining the dataset?} The authors will be supporting, hosting, and maintaining the dataset. 

\paragraph{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?} Please contact Qing Li (\texttt{liqing@bigai.ai}).

\paragraph{Is there an erratum?} No. We will make announcements if there is any. 

\paragraph{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?} Yes. New updates will be posted on \url{https://mm-fire.github.io/}.

\paragraph{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were the individuals in question told that their data would be retained for a fixed period of time and then deleted)?} The images in our dataset might contain human subjects, but all of them are from public datasets.

\paragraph{Will older versions of the dataset continue to be supported/hosted/maintained?} Yes, old versions will be permanently accessible on \href{https://huggingface.co}{huggingface.co}.

\paragraph{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?} Yes, please refer to \url{https://mm-fire.github.io/}.

\subsection{Composition}

\paragraph{What do the instances that comprise the dataset represent?} 
Our data is generally stored in the json files. Every instance includes the path of an image and the feedback-reflecting dialogues.

\paragraph{How many instances are there in total (of each type, if appropriate)?} There are 1.2M samples (1.1M for training set, 0.1M for test set), among which 200K are GPT-4V generated data, while the rests are simulated via the \model and \model-FD.

\paragraph{Does the dataset contain all possible instances or is it a sample
(not necessarily random) of instances from a larger set?} We provide all instances in our Huggingface data repositories. 

\paragraph{Is there a label or target associated with each instance?} Yes.

\paragraph{Is any information missing from individual instances?} No. 

\paragraph{Are relationships between individual instances made explicit
(e.g., users’ movie ratings, social network links)?} No.

\paragraph{Are there recommended data splits (e.g., training, development/validation,
testing)?} Yes. FIRE-100K and FIRE-1M are used for training and FIRE-Bench is used for testing.

\paragraph{Are there any errors, sources of noise, or redundancies in the
dataset?} Please refer to the limitations  in ~\cref{sec:conclusion}.

\paragraph{Is the dataset self-contained, or does it link to or otherwise rely on
external resources (e.g., websites, tweets, other datasets)?} The dataset is self-contained.

\paragraph{Does the dataset contain data that might be considered confidential?} No. 

\paragraph{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?} No.

\subsection{Collection Process}

The collection procedure, preprocessing, and cleaning are explained in detail in Section 2 of the main paper.

\paragraph{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?} 

All data collection, curation, and filtering are done by FIRE coauthors. 

\paragraph{Over what timeframe was the data collected?} The data was collected between Jan. 2024 and May 2024.

\subsection{Uses}
\paragraph{Has the dataset been used for any tasks already?} 
Yes, we have used FIRE for training our VLMs,  including \vicunamodel, \studentmodel, \model, \model-FD.

\paragraph{What (other) tasks could the dataset be used for?} Our dataset is primarily for facilitating research in enhancing the feedback-reflecting ability of VLMs. Our data might also be used to benchmark existing and future VLMs.

\paragraph{Is there anything about the composition of the dataset or the way
it was collected and preprocessed/cleaned/labeled that might impact future uses?}  No.

\paragraph{Are there tasks for which the dataset should not be used?}  We strongly oppose any research that intentionally generates harmful or toxic content using our data. 


\section{Data source}

Our dataset uses images from 27 diverse sources to provide a robust training dataset for FIRE. All 27 datasets are public datasets, and all the images can be downloaded via links in \cref{tab:supp-datasource}. The comprehensive list of the source datasets and links to their metadata are detailed below:

\begin{table}[h]
\caption{Data utilized from 27 source datasets for training and test data in FIRE.}
\label{tab:supp-datasource}
\centering
\resizebox{1\columnwidth}{!}{
% \setlength{\tabcolsep}{9pt}
\begin{tabular}{ c c c c c   }
\toprule 
 \href{https://huggingface.co/datasets/liuhaotian/LLaVA-Instruct-150K}{LLaVA}~\cite{llava} 
& \href{https://cocodataset.org/}{COCO}~\cite{lin2014microsoft}
& \href{https://segment-anything.com/dataset/index.html}{SAM}~\cite{kirillov2023segment} 
& \href{https://visualqa.org/}{VQAV2}~\cite{goyal2017making} 
& \href{https://cs.stanford.edu/people/dorarad/gqa/about.html}{GQA}~\cite{hudson2019gqa}  \\

\hline
 \href{https://homes.cs.washington.edu/~ranjay/visualgenome/index.html}{VG}~\cite{krishna2017visual} 
& \href{https://drive.google.com/drive/folders/1tCUQ-sq6vdshZVkF0ZeF3K4eztkXJgax}{Web-Celebrity}~\cite{chen2023sharegpt4v} 
& \href{https://drive.google.com/drive/folders/1tCUQ-sq6vdshZVkF0ZeF3K4eztkXJgax}{Web-Landmark}~\cite{chen2023sharegpt4v} 
& \href{https://drive.google.com/drive/folders/1tCUQ-sq6vdshZVkF0ZeF3K4eztkXJgax}{WikiArt}~\cite{saleh2015large} 
& \href{https://github.com/FreedomIntelligence/ALLaVA}{ALLaVA-Vflan}~\cite{chen2024allava}  \\

\hline
 \href{https://github.com/vis-nlp/ChartQA}{ChartQA}~\cite{masry2022chartqa} 
& \href{https://www.docvqa.org/}{DocVQA}~\cite{mathew2021docvqa} 
& \href{https://kushalkafle.com/projects/dvqa.html}{DVQA}~\cite{kafle2018dvqa} 
& \href{https://github.com/chen-judge/GeoQA}{GeoQA+}\cite{chen2021geoqa} 
& \href{https://huggingface.co/datasets/naver-clova-ix/synthdog-en}{Synthdog-EN}\cite{kim2022ocr}  \\

\hline
\href{https://huggingface.co/datasets/liuhaotian/llava-bench-in-the-wild}{LLaVA-in-the-Wild}~\cite{llava}
& \href{https://mmmu-benchmark.github.io/}{MMMU}~\cite{yue2023mmmu} 
& \href{https://github.com/QwenLM/Qwen-VL/blob/master/eval_mm/mme/EVAL_MME.md}{MME}~\cite{fu2024mme} 
& \href{https://github.com/yuweihao/MM-Vet}{MM-Vet}~\cite{yu2023mm} 
& \href{https://github.com/AILab-CVC/SEED-Bench}{SEED-bench}~\cite{li2023seed}  \\
\hline
\href{https://ocr-vqa.github.io/}{OCRVQA}~\cite{mishra2019ocr} 
& \href{https://textvqa.org/}{TextVQA}~\cite{singh2019towards} 
& \href{https://drive.google.com/drive/folders/1tCUQ-sq6vdshZVkF0ZeF3K4eztkXJgax}{Share-TextVQA}~\cite{chen2023sharegpt4v} 
& \href{https://allenai.org/data/diagrams}{AI2D}~\cite{kembhavi2016diagram} 
& \href{https://mathverse-cuhk.github.io/}{MathVerse}~\cite{zhang2024mathverse} \\
\hline
\href{https://mathvista.github.io/}{MathVista}~\cite{lu2023mathvista} 
&\href{https://scienceqa.github.io/}{ScienceQA}~\cite{lu2022scienceqa} 
\\

\bottomrule
\end{tabular}
}
\end{table}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


